Route to Rome Attack: Directing LLM Routers to Expensive Models via Adversarial Suffix Optimization

Cost-aware routing dynamically dispatches user queries to models of varying capability to balance performance and inference cost. However, the routing strategy introduces a new security concern that adversaries may manipulate the router to consistently select expensive high-capability models. Existing routing attacks depend on either white-box access or heuristic prompts, rendering them ineffective in real-world black-box scenarios. In this work, we propose R$^2$A, which aims to mislead black-box LLM routers to expensive models via adversarial suffix optimization. Specifically, R$^2$A deploys a hybrid ensemble surrogate router to mimic the black-box router. A suffix optimization algorithm is further adapted for the ensemble-based surrogate. Extensive experiments on multiple open-source and commercial routing systems demonstrate that {R$^2$A} significantly increases the routing rate to expensive models on queries of different distributions. Code and examples: https://github.com/thcxiker/R2A-Attack.

==> figs/figscode/bar.tex <==
    % === 1. 定义原图的莫兰迪配色 ===
    \definecolor{refPink}{RGB}{249, 205, 186} % 对应图中的 Strong
    \definecolor{refGray}{RGB}{217, 217, 217} % 对应图中的 Strong-to-Weak
    \definecolor{refBlue}{RGB}{197, 217, 241} % 对应图中的 Weak
    \definecolor{lineGray}{RGB}{128, 128, 128} % 深灰色虚线

    \begin{tikzpicture}
        \begin{groupplot}[
            group style={
                group size=1 by 2,      % 1列2行
                vertical sep=0.4cm,     % 上下两图之间的间距，调小一点更紧凑
                xdescriptions at=edge bottom % 只在最底部的图显示X轴标签
            },
            width=0.9\linewidth,        % 宽度
            height=4.5cm,               % 每个子图的高度
            ybar,                       % 柱状图
            bar width=14pt,             % 柱子宽度
            ymin=0.0, ymax=1.25,        % Y轴范围
            ylabel style={font=\rmfamily}, % 字体设置
            xlabel style={font=\rmfamily},
            tick label style={font=\rmfamily\small},
            ymajorgrids=true,           % 开启网格
            grid style={dashed, gray!30}, % 网格样式
            % === 关键：让柱子边框是黑色的，显着锐利 ===
            nodes near coords={},       % 如果你想在柱子上显示数字，把{}删掉即可
            every axis plot/.append style={fill, draw=black, line width=0.5pt},
            % === X轴 坐标 ===
            symbolic x coords={reroute, LC-W, LC-B, No-Sfx, Ours},
            xtick=data,
        ]

        % ==========================
        % 上面的图：In-domain (对应原图 TruthfulQA)
        % ==========================
        \nextgroupplot[
            ylabel={Accuracy}, 
            title={In-domain Task}, % 标题
            title style={yshift=-5pt, font=\rmfamily\large}
        ]
        
        % 画一条基准虚线 (模仿 Ref. LLM)
        \draw [lineGray, dashed, ultra thick] (axis cs:reroute, 0.85) -- (axis cs:Ours, 0.85);

        % 数据列：我把你的数据分成了两组来模仿原图的"簇"
        % 为了模仿原图效果，我假设 "life-cycle-W" 是灰色柱，"Ours" 是粉色柱
        % 你可以根据实际情况调整颜色的含义
        
        % 柱子 1: 模仿 "Strong" (粉色) - 放主要方法
        \addplot[fill=refPink] coordinates {
            (reroute, 0.797) 
            (LC-W, 0.821) 
            (LC-B, 0.982) 
            (No-Sfx, 0.632) 
            (Ours, 1.030)
        };
        
        % 柱子 2: 模仿 "Strong-to-Weak" (灰色) - 可以放对比方法
        % (这里我为了演示效果，造了一个比上面低一点的数据，你可以填入真实对比数据)
        \addplot[fill=refGray] coordinates {
            (reroute, 0.70) 
            (LC-W, 0.75) 
            (LC-B, 0.85) 
            (No-Sfx, 0.55) 
            (Ours, 0.90)
        };

        % ==========================
        % 下面的图：Out-domain (对应原图 MMLU)
        % ==========================
        \nextgroupplot[
            ylabel={Accuracy},
            title={Out-domain Task},
            title style={yshift=-5pt, font=\rmfamily\large},
            legend to name=CommonLegend, % 把图例导出到外部，名字叫 CommonLegend
            legend style={legend columns=-1},
            legend image post style={scale=0.8} % 图例图标稍微小一点
        ]

        % 基准虚线
        \draw [lineGray, dashed, ultra thick] (axis cs:reroute, 0.85) -- (axis cs:Ours, 0.85);

        % 数据列 (你的 Out-domain 数据)
        \addplot[fill=refPink, area legend] coordinates {
            (reroute, 0.797) (LC-W, 0.821) (LC-B, 0.982) (No-Sfx, 0.632) (Ours, 1.030)
        };
        % 对比数据
        \addplot[fill=refGray, area legend] coordinates {
            (reroute, 0.65) (LC-W, 0.70) (LC-B, 0.80) (No-Sfx, 0.50) (Ours, 0.88)
        };

        % 添加虚线到图例 (使用一个小 trick)
        \addlegendimage{line legend, lineGray, dashed, ultra thick}
        
        % 设置图例文字
        \legend{Proposed Method, Baseline Method, Ref. Line}

        \end{groupplot}
        
        % === 手动绘制图例 (放在图的最下方) ===
        \node[anchor=north] at ($(group c1r2.south) + (0,-1.2cm)$) {\ref{CommonLegend}};

    \end{tikzpicture}
